Exact Parallel Waves in General Relativity

We conduct a review of the basic definitions and the principal results in the study of wavelike spacetimes, that is spacetimes whose metric models massless radiation moving at the speed of light, focusing in particular on those geometries with parallel rays. In particular, we motivate and connect their various definitions, outline their coordinate descriptions and present some classical results in their study in a language more accessible to modern readers, including the existence of "null coordinates" and the construction of Penrose limits. We also present a thorough summary of recent work on causality in pp-waves, and describe progress in addressing an open question in the field - the Ehlers-Kundt conjecture.

==> media/FigureTemplates.tex <==
%--------------REGULAR IMAGE---------------
\iffalse

\begin{figure}
    \centering 
    \includegraphics[width=0.6\textwidth]{IMAGE.png}
    \caption{}
    \label{fig:LABEL}
\end{figure} 


%-------------HORIZONTAL ARRAY----------------

\begin{figure}%
\centering
\subfigure[Image A]{%
\label{fig:A}%
\includegraphics[width=0.45\textwidth]{A.png}}%
\qquad
\subfigure[Image B]{%
\label{fig:B}%
\includegraphics[width=0.45\textwidth]{B.png}}%
\caption{}
\label{fig:WholeFigureRef}
\end{figure}


%-------------2D ARRAY----------------

\begin{figure}%
    \centering
    \subfigure[Cap1]{%
        \label{fig:1}%
        \includegraphics[width=0.46\textwidth]{1.png}}%
    \qquad
    \subfigure[Cap2]{%
        \label{fig:2}%
        \includegraphics[width=0.46\textwidth]{2.png}}%
 \vskip\baselineskip
     \subfigure[Cap3]{%
        \label{fig:3}%
        \includegraphics[width=0.46\textwidth]{3.png}}%
    \qquad
    \subfigure[Cap4]{%
        \label{fig:4}%
        \includegraphics[width=0.46\textwidth]{4.png}}%
\caption{Caption of the whole thing}
\label{fig:2Darray}
\end{figure}

\fi
